TPA: Fast, Scalable, and Accurate Method for Approximate Random Walk with Restart on Billion Scale Graphs

Given a large graph, how can we determine similarity between nodes in a fast and accurate way? Random walk with restart (RWR) is a popular measure for this purpose and has been exploited in numerous data mining applications including ranking, anomaly detection, link prediction, and community detection. However, previous methods for computing exact RWR require prohibitive storage sizes and computational costs, and alternative methods which avoid such costs by computing approximate RWR have limited accuracy. In this paper, we propose TPA, a fast, scalable, and highly accurate method for computing approximate RWR on large graphs. TPA exploits two important properties in RWR: 1) nodes close to a seed node are likely to be revisited in following steps due to block-wise structure of many real-world graphs, and 2) RWR scores of nodes which reside far from the seed node are proportional to their PageRank scores. Based on these two properties, TPA divides approximate RWR problem into two subproblems called neighbor approximation and stranger approximation. In the neighbor approximation, TPA estimates RWR scores of nodes close to the seed based on scores of few early steps from the seed. In the stranger approximation, TPA estimates RWR scores for nodes far from the seed using their PageRank. The stranger and neighbor approximations are conducted in the preprocessing phase and the online phase, respectively. Through extensive experiments, we show that TPA requires up to 3.5x less time with up to 40x less memory space than other state-of-the-art methods for the preprocessing phase. In the online phase, TPA computes approximate RWR up to 30x faster than existing methods while maintaining high accuracy.

==> ICDM_legacy.tex <==
%TODO%%%%%%%%%%%%%%%%%%%%%%%Experiemnt%%%%%%%%%%%%%%%%%%%%
{\bfseries {\item Q2 Effectiveness of two approximate phases in \methodA.}}
How effective is the stranger approximation in terms of accuracy? (Section~\ref{sec:exp-stranger-approx})
How effective is the neighbor approximation in terms of accuracy? (Section~\ref{sec:exp-neighbor-approx})

\begin{figure}[!t]
	\centering
	\includegraphics[width=.7\linewidth]{FIG/FINAL/LEGEND_TPA_SMALL}\\
	\includegraphics[width=.85\linewidth]{FIG/FINAL/TPA_ACCURACY_L1}
	\vspace{-1mm}		
	\caption{
		L1 norm accuracy of \methodA:  
		we compare L1 norm of error of RWR score vectors of TPA and other methods {\color{blue}with regard to the exact RWR score vector.}
		\methodA provides the highest L1 norm accuracy among all tested methods. 
		Bars are omitted if corresponding experiments run {\color{blue}out of memory ($>200$GB).}
	}
	\label{fig:perf:tpa:l1_error}
	\centering
	\includegraphics[width=.85\linewidth]{FIG/FINAL/TPA_ACCURACY_RANK}
	\vspace{-4mm}			
	\caption{
		Rank accuracy of \methodA: \methodA shows the highest rank accuracy among competitors. The higher the Spearman correlation, the higher is the accuracy.
	}
	\label{fig:perf:tpa:acc:spearman}
\end{figure}

In many applications of RWR, one common approach is to return the ranking in vertices of RWR vector.
For example, in Twitter's "Who to Follow" recommendation service, the top-ranked users in RWR will be recommended.
On the other hand, for the trolling detection, the low-ranked users will be returned.
Therefore, it is important to measure the ranking error to examine the accuracy of an approximate RWR vector.
We use Spearman correlation~\cite{artusi2002bravais} which measures the similarity between two ranking vectors.
Note that the higher the Spearman correlation, the higher is the accuracy.
We also compare $L1$ norm error between an approximate RWR vector and its true RWR vector.
As shown in Figures~\ref{fig:perf:tpa:l1_error} and \ref{fig:perf:tpa:acc:spearman}, \methodA outperforms other state-of-the-art methods with higher accuracy by up to $9\times$ in $L1$ norm and $2\times$ in ranking.
Note that {\color{blue}\methodA does not require more computation time or memory to achieve higher accuracy than other methods.
	BEAR-APPROX needs $5923\times$ more preprocessing time than \methodA to achieve its best $L1$ accuracy which is similar with \methodA on the Google dataset.}
BRPPR needs $354\times$ more online time than \methodA to achieve its best ranking accuracy which is still $1.1\times$ lower than \methodA on the Friendster dataset. 
{\color{blue}HubPPR which achieves relatively higher $L1$ norm accuracy than other competitors requires more memory and more computation time for both phases than \methodA.}

\begin{figure}[!t]
	\centering
	\vspace{-2mm}
	\includegraphics[width=.67\linewidth]{FIG/FINAL/STR_LEGEND}\\
	\vspace{-0.5mm}
	\hspace{-5mm}
	\subfigure[L1 norm of error]
	{
		\includegraphics[width=.49\linewidth]{FIG/FINAL/TPA_STRANGER_L1}
		\vspace{-4mm}
	}
	\hspace{-5mm}
	\subfigure[Spearman correlation]
	{
		\includegraphics[width=.49\linewidth]{FIG/FINAL/TPA_STRANGER_RANK}
		\vspace{-4mm}			
	}
	\vspace{-1mm}
	\caption
	{
		Effectiveness of the stranger approximation:
		with the help of the stranger approximation, \methodA shows higher accuracy than \methodAN, especially in ranking. 
	}
	\label{fig:perf:stranger}
\end{figure}
\begin{figure}[!t]
	\centering
	\vspace{-2mm}
	\hspace{-2mm}
	\includegraphics[width=.67\linewidth]{FIG/FINAL/NB_LEGEND}\\
	\hspace{-5mm}
	\subfigure[L1 norm of error]
	{
		\includegraphics[width=.49\linewidth]{FIG/FINAL/TPA_NB_L1}
		\vspace{-4mm}
	}
	\hspace{-5mm}
	\subfigure[Spearman correlation]
	{
		\includegraphics[width=.49\linewidth]{FIG/FINAL/TPA_NB_RANK}
		\vspace{-8mm}			
	}
	\vspace{-1mm}
	\caption
	{
		Effectiveness of the neighbor approximation:
		\methodAN on real-world graphs shows lower $L1$ error and higher rank error than \methodAN on random graphs. 
	}
	\label{fig:perf:neighbor}
\end{figure}

\subsection{Effectiveness of Stranger Approximation}
\label{sec:exp-stranger-approx}

To examine the effectiveness of the stranger approximation, we define a new term $\r_{\text{\methodAN}}$ {\color{blue}which omits the stranger approximation $\rtilde_{\text{stranger}}$ from $\r_{\text{\methodA}}$} as follows:
\begin{align*}
\r_{\text{\methodAN}} = \r_{\text{family}} + \rtilde_{\text{neighbor}}
\end{align*}
We compare $\r_{\text{\methodA}}$ with $\r_{\text{\methodAN}}$ in terms of accuracy.
In Figure~\ref{fig:perf:stranger}, $\r_{\text{\methodA}}$ shows higher accuracy than $\r_{\text{\methodAN}}$, especially in ranking.
Without the stranger approximation, $\r_{\text{\methodAN}}$ has no information to estimate RWR scores of nodes far from the seed;
and thus, the scores of the faraway nodes are totally ignored.
With the help of the stranger approximation, $\r_{\text{TPA}}$ succeeds in estimating RWR scores of the nodes far from the seed, thus enhancing the overall RWR accuracy.
{\color{blue}The reason for the small improvements in $L1$ error by the stranger approximation is that $L1$ norm of $\rtilde_{\text{stranger}}$ is relatively small, and thus affects insignificantly on the total $L1$ error.}

\subsection{Effectiveness of Neighbor Approximation}
\label{sec:exp-neighbor-approx}

To examine the effectiveness of the neighbor approximation, we measure the accuracy of the neighbor approximation on real-world graphs, and compare it with the accuracy of the neighbor approximation on random graphs.
Random graphs have the same numbers of nodes and edges with their corresponding real-world graphs, but their edges are randomly distributed.
Since the main idea of the neighbor approximation is based on block-wise structure of real-world graphs, the random distribution of edges in random graphs would not see the accuracy improvements by the neighbor approximation.
We estimate the accuracy of $\r_{\text{\methodAN}}$ on both types of graphs since $\r_{\text{\methodAN}}$ includes the effect of the neighbor approximation solely.
In Figure~\ref{fig:perf:neighbor}, we observe that $\r_{\text{\methodAN}}$ on real-world graphs shows higher $L1$ norm accuracy than $\r_{\text{\methodAN}}$ on random graphs.
This shows that the neighbor approximation works effectively on real-world graphs. 
On the other hand, $\r_{\text{\methodAN}}$ on real-world graphs shows low ranking accuracy.
This is also due to block-wise structure of real-world graphs:
random graphs have more out-edges escaped from a community, hence $\r_{\text{\methodAN}}$ has more chance to consider nodes from different communities, while block-wise structure of real-world graphs prevents $\r_{\text{\methodAN}}$ to consider nodes in other communities. 
Note that \methodA complements the low ranking accuracy of \methodAN with the help of the stranger approximation; 
TPA's RWR score vector $\r_{\text{\methodA}}$ gives much higher Spearman correlation than $\r_{\text{\methodAN}}$ does as shown in Figure~\ref{fig:perf:stranger}. 


%TODO%%%%%%%%%%%%%%%%%%%%%%%PRELIMINARY%%%%%%%%%%%%%%%%%%%
\subsection{Power Iteration}\label{sec:pi}
Among various PageRank and RWR computation methods~\cite{kamvar2003exploiting, kamvar2004adaptive, haveliwala1999efficient}, the power iteration (PI)~\cite{page1999pagerank} is most widely used in graph engines~\cite{cheng2015venus, gonzalez2012powergraph, gonzalez2014graphx, malewicz2010pregel}.
PI repeatedly computes its iterative equations (Equations~\eqref{eq:pagerank} and~\eqref{eq:rwr}) until convergence to get the answer.
The iterative equation for PageRank is defined as follows:

\begin{theorem}
	\label{theorem:accurate_cpi}
	Let $\r_{\text{PI}}$ be the true solution of the recursive equation $\r = (1-c)\NAT\r + c\q$ computed by the power iteration (PI).
	Then $\r_{\text{\methodE}}$ equals $\r_{\text{PI}}$.
	\begin{IEEEproof}
		The procedure of PI is represented as follows:
		\begin{align*}
		\r_{\text{PI}}^{(i)} &= (1-c)\NAT\r_{\text{PI}}^{(i-1)} + c\q \\
		&= \left((1-c)\NAT\right)^{2}\r_{\text{PI}}^{(i-2)} + c\left((1-c)\NAT + \mat{I}\right)\q \\
		&= \cdots \\
		&= \left((1-c)\NAT\right)^{i}\r_{\text{PI}}^{(0)} + c\left(\sum_{j=0}^{i-1}\left((1-c)\NAT\right)^{j}\right)\q
		\end{align*}	
		If $i \rightarrow \infty$, then the above equation is represented as the following equation:
		\begin{align*}
		\lim_{i \rightarrow \infty}\r_{\text{PI}}^{(i)} = c\left(\sum_{j=0}^{\infty}\left((1-c)\NAT\right)^{j}\right)\q = \r_{\methodE}
		\end{align*}
		\noindent Note that the spectral radius of $(1-c)\NAT$ is less than one since $\NAT$ is a column stochastic matrix, which implies that $\lim_{i \rightarrow \infty}((1-c)\NAT)^{i} = \mat{0}$.
		Thus, $\r_{\methodE} = \r_{\text{PI}}$.
	\end{IEEEproof}
\end{theorem}
%TODO%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  TPA   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this section, we describe our proposed method TPA-RWR for fast, memory-efficient, and highly accurate approximate RWR computation based on \methodE. %, a new iterative method for RWR computation.

\subsection{Overview}
\label{subsec:overview}

\methodE interprets RWR as propagation of score $c$ from a seed node across the graph.
{\color{blue}
	In \methodE, $i$-th iteration computes propagation of scores across nodes at $i$-th steps from the seed node.
	After one iteration finishes, propagation of scores goes one step further.
}
\methodA divides the propagation process, the whole iterations in \methodE into three parts as follows:
\begin{align*}
\r_{\text{CPI}} = \r_{\text{family}} + \r_{\text{neighbor}} + \r_{\text{stranger}}
\end{align*}

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.9\linewidth]{FIG/FINAL/FLOW}
	%\vspace{1mm}
	\caption{
		Overview: \methodA divides \methodE into three parts and applies the neighbor approximation and the stranger approximation on the neighbor part and the stranger part, respectively.
	}
	\label{fig:tpa:flow}
	\vspace{1mm}
\end{figure}

$S$ denotes the starting iteration in $\r_{\text{neighbor}}$, and $T$ denotes the starting iteration in $\r_{\text{stranger}}$.
The family part $\r_{\text{family}}$ denotes the propagation of scores into nearby nodes from the seed and comprises the iterations from $0$th to ($S-1$)th in \methodE.
The neighbor part  $\r_{\text{neighbor}}$ denotes the propagation following the family part and comprises the iterations from $S$th to ($T-1$)th.
Finally, the rest propagation part, the iterations from $T$th to the end, is denoted as $\r_{\text{stranger}}$.
%To reach the stranger part, we need long steps from the seed thus naming 'stranger' to the part.
Based on this partition, \methodA approximates $\r_{\text{neighbor}}$ and $\r_{\text{stranger}}$ by the neighbor approximation phase and the stranger approximation phase, respectively.
In the stranger approximation phase, \methodA estimates $\r_{\text{stranger}}$ using PageRank.
In the neighbor approximation phase, \methodA approximates $\r_{\text{neighbor}}$ using $\r_{\text{family}}$ which is the only part computed exactly.
Then the neighbor approximation and the stranger approximation are merged in finalizing phase.
The main ideas of our proposed method are summarized as follows:

\begin{itemize}
	%\item{
	%	\textbf{\methodE}
	%	represents the propagation of scores on a given graph and accumulates the propagated scores at each node during iterations to get the final RWR score (Section~\ref{subsec:cpi}).
	%}
	\item{
		\textbf{\methodA: stranger approximation}
		approximates the stranger part $\r_{\text{stranger}}$ in RWR with the stranger part $\p_{\text{neighbor}}$ in PageRank based on the observation that scores computed in the stranger part are highly affected by distribution of the given graph regardless of the seed node (Section~\ref{subsec:stranger_approx}).
	}
	\item{
		\textbf{\methodA: neighbor approximation}
		approximates the neighbor part $\r_{\text{neighbor}}$ using the family part $\r_{\text{family}}$ taking the advantage of block-wise structure of many real-world graphs (Section~\ref{subsec:neighbor_approx}).
	}
\end{itemize}
%After elaborating \methodE algorithm (Section~\ref{subsec:cpi}), 
{\color{blue}
	We describe \methodA algorithm with its accuracy analysis (Section~\ref{subsec:tpa}), and analyze time and space complexities (Section~\ref{subsec:tpa-performance}).
}


%TODO%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  Strager Approximation %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Accuracy analysis.} We show the accuracy bound of $\rtilde_{\text{stranger}}$ in Lemma~\ref{lemma:bound_stranger} using Lemma~\ref{lemma:bound_ith_stranger}.
\begin{lemma}
	\label{lemma:bound_ith_stranger}
	L1 norm of the error between RWR interim score vector $\x^{(i)}$ and PageRank interim score vector $\x'^{(i)}$ at $i$th iteration in $\methodE$ is bounded as follows:
	$\lVert \x^{(i)} - \x'^{(i)}\rVert_{1} \leq 2c(1-c)^{i}$
	\begin{IEEEproof}
		The interim score vectors $\x^{(i)}$ and $\x'^{(i)}$ at $i$-th iteration in \methodE are represented as follows:
		\begin{align*}
		\x^{(i)} = (1-c)\NAT\x^{(i-1)} = c(1-c)^{i}(\NAT)^{i}\q \\
		\x'^{(i)} = (1-c)\NAT\x'^{(i-1)} = c(1-c)^{i}(\NAT)^{i}\vect{b}	
		\end{align*}
		\noindent where $\q$ is $s$-th unit vector, and $\vect{b} = \frac{1}{n}\vect{1}$.
		%Suppose $(\NAT)^{i}$ is represented by $\begin{bmatrix}
		%\vect{c}_{1}, \cdots, \vect{c}_{n}
		%\end{bmatrix}$ where $\vect{c}_{j}$ is $j$-th column of the matrix, and $n$ is the number of nodes.
		Then, $\x^{(i)} - \x'^{(i)}$ is represented as follows:
		\begin{align*}
		\x^{(i)} - \x'^{(i)} = c(1-c)^{i}(\NAT)^{i}(\q - \vect{b})
		%&= c(1-c)^{i}(\vect{c}_{s} - \frac{1}{n}\vect{c}_{1} - \cdots - \frac{1}{n}\vect{c}_{n}) \\
		%&= \frac{c(1-c)^{i}}{n}\sum_{j \neq s}(\vect{c}_{s}-\vect{c}_{j})
		\end{align*}
		Then, $\lVert \x^{(i)} - \x'^{(i)}\rVert_{1}$ is bounded by the following inequality:
		\begin{align*}
		\lVert \x^{(i)} - \x'^{(i)}\rVert_{1} &= \lVert c(1-c)^{i}(\NAT)^{i}(\q - \vect{b})\rVert_{1}\\
		&\leq c(1-c)^{i}\lVert \q - \vect{b}\rVert_{1}\\
		&= c(1-c)^{i}\frac{2(n-1)}{n}\\
		&\leq 2c(1-c)^{i}
		%\lVert \x^{(i)} - \x'^{(i)}\rVert_{1} &= \frac{c(1-c)^{i}}{n}\lVert \sum_{j \neq s}(\vect{c}_{s}-\vect{c}_{j}) \rVert_{1} \\
		%&\leq \frac{c(1-c)^{i}}{n}\sum_{j \neq s}\lVert\vect{c}_{s}-\vect{c}_{j} \rVert_{1}\\
		%&\leq \frac{c(1-c)^{i}}{n}\times 2(n-1) \leq 2c(1-c)^{i}
		\end{align*}
		where the first inequality comes from the property of sub-multiplicative property of L1 norm.
		Note that $\lVert (\NAT)^{i} \rVert_{1} = 1$ since $\NAT$ is a column stochastic matrix; thus, $(\NAT)^{i}$ is also a column stochastic matrix.
		%Note that $\lVert \vect{c}_{j} \rVert_{1} \leq 1$ since $\lVert \NAT \rVert_{1} = 1$ and $\lVert (\NAT)^{t} \rVert_{1} \leq \lVert \NAT \rVert_{1}^{t} = 1$; thus, the inequality $\lVert \vect{c}_{j} \rVert_{1} \leq 1$ implies that $\lVert \vect{c}_{s} - \vect{c}_{j} \rVert_{1} \leq \lVert \vect{c}_{s} \rVert_{1} + \lVert \vect{c}_{j} \rVert_{1} \leq 2$.	
	\end{IEEEproof}
\end{lemma}
\begin{lemma}[Accuracy bound for $\rtilde_{\text{stranger}}$]
	\label{lemma:bound_stranger}
	Let $\r_{\text{stranger}}$ be the exact stranger part in \methodE, $\rtilde_{\text{stranger}}$ be the approximate stranger part via the stranger approximation, and $T$ be the starting iteration of the stranger part. Then $\lVert \r_{\text{stranger}} - \rtilde_{\text{stranger}} \rVert_{1} \leq 2(1-c)^{T}$.
	\begin{IEEEproof}
		$\r_{\text{stranger}}$ and $\rtilde_{\text{stranger}}$ are represented as follows:
		\begin{align*}
		\r_{\text{stranger}}&= \x^{(T)} + \x^{(T+1)} + \cdots \\
		\rtilde_{\text{stranger}} &= \x'^{(T)} + \x'^{(T+1)} + \cdots
		\end{align*}
		Then, $\lVert \r_{\text{stranger}} - \rtilde_{\text{stranger}}  \rVert_{1}$ is bounded as follows:
		\begin{align*}
		\lVert \r_{\text{stranger}} - \rtilde_{\text{stranger}}  \rVert_{1} &= \lVert \x^{(T)} + \cdots - (\x'^{(T)} + \cdots) \rVert_{1} \\
		&\leq \sum_{i=T}^{\infty} \lVert \x^{(i)} - \x'^{(i)} \rVert_{1}
		\leq 2c\sum_{i=T}^{\infty} (1-c)^{i} \\
		&=2c\times\frac{(1-c)^{T}}{c} = 2(1-c)^{T}
		\end{align*}
		Note that $\lVert \x^{(i)} - \x'^{(i)} \rVert_{1} \leq 2c(1-c)^{i}$ by Lemma~\ref{lemma:bound_ith_stranger}.
	\end{IEEEproof}
\end{lemma}


%TODO%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  Neighbor Approximation %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The bound of $\lVert \rnb - \trnb \rVert_{1}$ is represented as follows:
\begin{align*}
\lVert \rnb - \trnb \rVert_{1} &\leq \lVert \rnb \rVert_{1} + \lVert \trnb \rVert_{1}\\
&= \lVert \rnb \rVert_{1} + \frac{\lVert \rnb \rVert_{1}}{\lVert \rfm \rVert_{1}}\lVert \rfm \rVert_{1}\\
&= 2\lVert \rnb \rVert_{1} \\
&= 2(1-c)^{S} - 2(1-c)^{T}
\end{align*}
Note that $\lVert \rnb \rVert_{1} = (1-c)^{S} - (1-c)^{T}$ by Lemma~\ref{lemma:neighbor length}.

%TODO omission Monte-Carlo method
%Unlike Monte-Carlo based RWR methods~\cite{fogaras2005towards, liu2016powerwalk} who select one out-edge of a node to follow randomly and calculate probability based on sampling, \methodE propagates scores into all out-edges.
%This contributes to the better approximation because possibility that propagation trajectories in faraway-neighbor iterations and close-neighbor iterations would overlap increases in \methodE.
%TODO add deadend explanation? or not?....
%In addition, we need to provide special handling for dead-ends to avoid unexpected results.
%In neighbor approximation phase, when neighbor queue $Queue$ is empty, it means that the current node is dead-end.
%Then, only neighbor approximation is merged to the final RWR value because there is no route to propagate scores into stranger iterations, thus stranger approximation is useless.
%Then, the final RWR score of each node is its accumulated scores as shown in Algorithm~\ref{alg:cpi}
%TODO Hub and Spoke
%To exploit block-wise structure, we need to consider two types of nodes, hub and spoke, which show different patterns in block-wise, community-like structure:
%spoke nodes present clear communities among them while hub nodes are not belonging to a specific community but connected with most of nodes in a graph~\cite{kang2011beyond}.
%For spoke nodes who have most out-edges directed into their own small communities, propagation trajectory in the family part would be overlapped by the following neighbor part.
%For hub nodes who have a lot of out-edges across the graph, \methodE iterations are expected to converge fast since their scores are divided and propagated into their high number of out-edges.
%In other words, RWR scores for hub nodes are determined by early iterations.
%Neighbor approximation shows high accuracy and effectiveness over hub and spoke in our experiment (Section~\ref{sec:exp-neighbor-approx}).
